Impact of Array Configuration on Head-Mounted Display Performance at mmWave Bands

Immersing a user in life-like extended reality (XR) scenery using a head-mounted display (HMD) with a constrained form factor and hardware complexity requires remote rendering on a nearby edge server or computer. Millimeter-wave (mmWave) communication technology can provide sufficient data rate for wireless XR content transmission. However, mmWave channels exhibit severe sparsity in the angular domain. This means that distributed antenna arrays are required to cover a larger angular area and to combat outage during HMD rotation. At the same time, one would prefer fewer antenna elements/arrays for a lower complexity system. Therefore, it is important to evaluate the trade-off between the number of antenna arrays and the achievable performance to find a proper practical solution. This work presents indoor 28 GHz mmWave channel measurement data, collected during HMD mobility, and studies the dominant eigenmode (DE) gain. DE gain is a significant factor in understanding system performance since mmWave channel sparsity and eigenmode imbalance often results in provisioning the majority of the available power to the DE. Moreover, it provides the upper performance bounds for widely-adopted analog beamformers. We propose 3 performance metrics - gain trade-off, gain volatility, and minimum service trade-off - for evaluating the performance of a multi-array HMD and apply the metrics to indoor 28 GHz channel measurement data. Evaluation results indicate, that 3 arrays provide stable temporal channel gain. Adding a 4th array further increases channel capacity, while any additional arrays do not significantly increase physical layer performance.

==> figure-journal/mobility-sequence/mobility_sequence.tex <==
\begin{tikzpicture}

\newcommand\imagewidth{1} % AP image width
\newcommand\pitchoffsety{3} % Y offset when pitched
\newcommand\axisoffsety{2.2} % Y offset of time axis below pithced
\newcommand\snapshotoffsety{0.1} % Y offset of snapshot count below time axis
\newcommand\dotsoffsetx{0.25} % Dots X offset on time axis

\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}


%%% BEGIN: DEVICES %%%

%%% Pre-define device positions for object placement

\node[] (ue_upright) at (1,5) {};
\node[] (ue_rotated1) at ([xshift=2.8 cm]ue_upright) {};
\node[] (ue_pitched) at ([xshift=0 cm, yshift=-\pitchoffsety cm]ue_rotated1) {};
\node[] (ue_rotated2) at ([xshift=2.8 cm]ue_pitched) {};
\node[] (ap) at (8.89-\imagewidth*0.5,5) {};


%%% UE

\node[black, anchor=south] at([yshift=(\imagewidth+0.0)*1cm]ue_rotated1.center) {\textbf{\underline{HMD}}};
\draw[thick] (ue_upright.center) -- ([yshift=-4cm]ue_upright.center);
\draw[thick] ([yshift=-3.5cm]ue_upright.center) --++ (-60:1cm);
\draw[thick] ([yshift=-3.5cm]ue_upright.center) --++ (-120:1cm);
\fill[black] ([yshift=-1.3cm]ue_upright.center) circle (1mm);

% Pitch axis
\draw[{angle 60}-{angle 60}] 
    ([xshift=-0.7\imagewidth cm, yshift=-0.1 cm]ue_upright.center) --
    ([xshift=-0.7\imagewidth cm, yshift=-1.3cm]ue_upright.center);
\draw[] 
    ([xshift=-(0.7\imagewidth-0.1)*1cm, yshift=-0.1 cm]ue_upright.center) --
    ([xshift=-(0.7\imagewidth+0.1)*1cm, yshift=-0.1 cm]ue_upright.center);
\draw[] 
    ([xshift=-(0.7\imagewidth-0.4)*1cm, yshift=-1.3 cm]ue_upright.center) --
    ([xshift=-(0.7\imagewidth+0.1)*1cm, yshift=-1.3 cm]ue_upright.center);
\node[anchor=south, rotate=90] at ([xshift=-(0.7\imagewidth)*1cm, yshift=-0.7 cm]ue_upright.center) {\SI{25}{\centi\meter}};

\node[align=center] (pithcaxistext) at ([xshift=+1.2cm, yshift=-2.2cm]ue_upright.center) {\footnotesize Pitch axis ($\beta$)};
\draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
    ([xshift=0.3cm,yshift=-1.3cm]ue_upright.center) 
    [partial ellipse=170:-170:0.075cm and 0.400cm]
;
\draw[black, dashed] ([xshift=-0.16cm, yshift=-1.3cm]ue_upright.center) --++(0.8cm,0);
\draw[-{angle 60}] ([xshift=0mm]pithcaxistext.north) to[out=90, in=-22] ([xshift=0.5cm, yshift=-1.45cm]ue_upright.center);

\node[align=center] (yawaxistext) at ([xshift=+1.2cm, yshift=-3.8cm]ue_upright.center) {\footnotesize Yaw axis ($\alpha$)};
% \draw[dashed] ([yshift=-2.3cm]ue_upright.center) ellipse (0.2cm and 0.8cm);
\draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
    ([yshift=-3.0cm]ue_upright.center) 
    [partial ellipse=255:-80:0.40cm and 0.075cm]
;
\draw[-{angle 60}] ([xshift=0mm]yawaxistext.north) to[out=90, in=-23] ([xshift=0.55cm, yshift=-3.07cm]ue_upright.center);

% UE size
\draw[{angle 60}-{angle 60}] 
    ([xshift=-0.5\imagewidth cm, yshift=(\imagewidth+0.1)*1cm]ue_upright.center) --
    ([xshift=+0.5\imagewidth cm, yshift=(\imagewidth+0.1)*1cm]ue_upright.center);
\foreach \xsign in {-1,1} {
    \draw[] 
    ([xshift=0.5*\xsign*\imagewidth*1cm, yshift=(\imagewidth-0.0)*1cm]ue_upright.center) --
    ([xshift=0.5*\xsign*\imagewidth*1cm, yshift=(\imagewidth+0.2)*1cm]ue_upright.center);
}
\node[anchor=south] at ([yshift=(\imagewidth+0.1)*1cm]ue_upright.center) {\SI{6}{\centi\meter}};


% Device pictures

\node[] at (ue_upright)
    {\includegraphics[width=\imagewidth cm]
    {figure-journal/mobility-sequence/ue_upright.png}
};

\node[] at (ue_rotated1)
    {\includegraphics[width=0.97\imagewidth cm]
    {figure-journal/mobility-sequence/ue_rotated1.png}
};

\node[] at (ue_pitched)
    {\includegraphics[width=\imagewidth cm]
    {figure-journal/mobility-sequence/ue_pitched.png}
};

\node[] at (ue_rotated2)
    {\includegraphics[width=1.5\imagewidth cm]
    {figure-journal/mobility-sequence/ue_rotated2.png}
};


% UE movement

\draw[-{angle 60}] ([xshift=0.7cm, yshift=-0.2cm]ue_upright.center) to[out=-20, in=-160] ([xshift=-0.7cm, yshift=-0.24cm]ue_rotated1.center);
\node[anchor=center] at ([xshift=1.45cm, yshift=-0.1cm]ue_upright.center) {\small $\alpha=30^{\circ}$};

\draw[-{angle 60}] ([yshift=-0.75cm]ue_rotated1.center) -- ([yshift=0.75cm]ue_pitched.center);
\node[anchor=center] at ([xshift=-0.65cm, yshift=-1.5cm]ue_rotated1.center) {\small $\beta=30^{\circ}$};

\draw[-{angle 60}] ([xshift=0.7cm, yshift=-0.7cm]ue_pitched.center) to[out=-20, in=-160] ([xshift=-0.7cm, yshift=-0.7cm]ue_rotated2.center);
\node[anchor=center] at ([xshift=1.45cm, yshift=-0.58cm]ue_pitched.center) {\small $\alpha=30^{\circ}$};


% UE coordinate systems

% \draw[ueRed, -{angle 60}] ([xshift=(+0.38\imagewidth)*1cm, yshift=-0.096cm]ue_upright.center) --++ (-55:0.45cm); % x (roll)
% \draw[ueRed, -{angle 60}] ([xshift=(+0.38\imagewidth)*1cm, yshift=-0.096cm]ue_upright.center) --++ (25:0.7cm); % y (pitch)
% \draw[ueRed, -{angle 60}] ([xshift=(+0.38\imagewidth)*1cm, yshift=-0.096cm]ue_upright.center) --++ (90:1.0cm); % z (yaw)
% \node[ueRed] at ([xshift=0.9cm, yshift=-0.7cm]ue_upright.center) {VII}; % x (roll)
\draw[ueRed, -{angle 60}] ([xshift=(-0.265\imagewidth)*1cm, yshift=-0.09cm]ue_upright.center) --++ (-125:0.45cm); % x (roll)
\draw[ueRed, -{angle 60}] ([xshift=(-0.265\imagewidth)*1cm, yshift=-0.09cm]ue_upright.center) --++ (-15:0.7cm); % y (pitch)
\draw[ueRed, -{angle 60}] ([xshift=(-0.265\imagewidth)*1cm, yshift=-0.09cm]ue_upright.center) --++ (90:1.0cm); % z (yaw)
\node[ueRed] at ([xshift=-0.48cm, yshift=-0.74cm]ue_upright.center) {\footnotesize VII};

\draw[ueRed, -{angle 60}] ([yshift=-0.12cm]ue_rotated1.center) --++ (-90:0.3cm); % x (roll)
\draw[ueRed, -{angle 60}] ([yshift=-0.12cm]ue_rotated1.center) --++ (0:1.0cm); % y (pitch)
\draw[ueRed, -{angle 60}] ([yshift=-0.12cm]ue_rotated1.center) --++ (90:1.0cm); % z (yaw)
\node[ueRed] at ([yshift=-0.55cm]ue_rotated1.center) {\footnotesize VII};

\draw[ueRed, -{angle 60}] ([yshift=-0.31cm]ue_pitched.center) --++ (-90:0.9cm); % x (roll)
\draw[ueRed, -{angle 60}] ([yshift=-0.31cm]ue_pitched.center) --++ (0:1.0cm); % y (pitch)
\draw[ueRed, -{angle 60}] ([yshift=-0.31cm]ue_pitched.center) --++ (90:0.5cm); % z (yaw)
\node[ueRed] at ([yshift=-1.36cm]ue_pitched.center) {\footnotesize VII};

\draw[ueRed, -{angle 60}] ([xshift=(0.2\imagewidth)*1cm, yshift=-0.37cm]ue_rotated2.center) --++ (-45:0.8cm); % x (roll)
\draw[ueRed, -{angle 60}] ([xshift=(0.2\imagewidth)*1cm, yshift=-0.37cm]ue_rotated2.center) --++ (30:0.45cm); % y (pitch)
\draw[ueRed, -{angle 60}] ([xshift=(0.2\imagewidth)*1cm, yshift=-0.37cm]ue_rotated2.center) --++ (45:0.65cm); % z (yaw)
\node[ueRed] at ([xshift=0.8cm, yshift=-1.1cm]ue_rotated2.center) {\footnotesize VII};



%%% AP

\node[black, anchor=south] at([yshift=(\imagewidth+0.0)*1cm]ap.center) {\textbf{\underline{AP}}};
\draw[thick] (ap.center) -- ([yshift=-4cm]ap.center);
\draw[thick] ([yshift=-3.5cm]ap.center) --++ (-60:1cm);
\draw[thick] ([yshift=-3.5cm]ap.center) --++ (-120:1cm);

\draw[{angle 60}-{angle 60}] 
    ([xshift=0.8\imagewidth cm, yshift=-0.1 cm]ap.center) -- 
    ([xshift=0.8\imagewidth cm, yshift=-4.2 cm]ap.center)
;
\foreach \yshift in {-0.1, -4.2}{
    \draw[] 
        ([xshift=(0.8\imagewidth-0.1)*1cm, yshift=\yshift cm]ap.center) -- 
        ([xshift=(0.8\imagewidth+0.1)*1cm, yshift=\yshift cm]ap.center);
}
\node[anchor=south, rotate=90] at([xshift=0.8\imagewidth cm, yshift=-2.1 cm]ap.center) {\SI{180}{\centi\meter}};


% Device picture

\node[] at (ap)
    {\includegraphics[width=1.2\imagewidth cm]
    {figure-journal/mobility-sequence/ap.png}
};

%%% END: DEVICES %%%


%%% BEGIN: LEGEND %%%

\draw[black, fill=white!90!black] (5, 2.95) rectangle ++(2.4, 3.5);


% UE top-down view

\def\xoffset{5.75}
\def\yoffset{5.15}
% \def\xoffset{4.7}
% \def\yoffset{2.6}

% \node[align=center, anchor=center] (td) at (\xoffset-0.15, \yoffset+1.4) {\footnotesize HMD top-down view};
% \draw[black, -{angle 60}] ([xshift=-0.5cm, yshift=-0.05cm]td.south) to[out=-90, in=150] ([xshift=-0.2cm, yshift=-0.35cm]td.south);

\draw [black, line width=0.5] 
(0.000 + \xoffset, 0.274 + \yoffset) --    
(0.000 + \xoffset, 0.574 + \yoffset) --
(0.274 + \xoffset, 0.848 + \yoffset) -- 
(0.574 + \xoffset, 0.848 + \yoffset) -- 
(0.848 + \xoffset, 0.574 + \yoffset) -- 
(0.848 + \xoffset, 0.274 + \yoffset) -- 
(0.574 + \xoffset, 0.000 + \yoffset) -- 
(0.274 + \xoffset, 0.000 + \yoffset) -- 
(0.000 + \xoffset, 0.274 + \yoffset);

\node [black] at (-0.20 + \xoffset, 0.424 + \yoffset) {\footnotesize V};
\node [black] at  (-0.08 + \xoffset, 0.798 + \yoffset) {\footnotesize IV};
\node [black] at  (0.424 + \xoffset, 1.048 + \yoffset) {\footnotesize III};
\node [black] at  (0.900 + \xoffset, 0.798 + \yoffset) {\footnotesize II};
\node [black] at (1.048 + \xoffset, 0.424 + \yoffset) {\footnotesize I};
\node [black] at  (1.050 + \xoffset, 0.050 + \yoffset) {\footnotesize VIII};
\node [red] at  (0.424 + \xoffset, -0.20 + \yoffset) {\footnotesize VII};
\node [black] at  (-0.08 + \xoffset, 0.050 + \yoffset) {\footnotesize VI};

\foreach \i in {-1, 1} {
    \draw [black, line width=1.0, fill=white!90!black] (0.424 + \i*0.25 + \xoffset, \yoffset+0.25) ellipse (0.2 and 0.1);
    \fill [black, line width=1.0] (0.424 + \i*0.25 + \xoffset, -0.05 + \yoffset+0.25) ellipse (0.1 and 0.05);
}
\draw [black, line width=1.0] (0.424 - 0.1 + \xoffset, -0.25 + \yoffset + 0.4) arc (-160:-20:0.1);



\node[] (vr_head) at (6.1,3.7)
    {\includegraphics[width=0.7\imagewidth cm]
    {figure-journal/mobility-sequence/vr_head.png}
};

\draw[black, -{angle 60}] ([xshift=-0.2cm, yshift=-0.2cm]vr_head.center) --++ (-135:0.5cm); % x (roll)
\node[black] at ([xshift=-0.75cm, yshift=-0.55cm]vr_head.center) {$x$};
\draw[black, -{stealth[length=1mm,width=1mm]}, rotate=-45] 
    ([xshift=-0.0cm, yshift=-0.45cm]vr_head.center) 
    [partial ellipse=440:100:0.20cm and 0.05cm]
;
\node[black] at ([xshift=-0.62cm, yshift=-0.17cm]vr_head.center) {$\gamma$};

\draw[black, -{angle 60}] ([xshift=0.40cm]vr_head.center) --++ (0:0.5cm); % y (pitch)
\node[black] at ([xshift=1.05cm, yshift=0.0cm]vr_head.center) {$y$};
\draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
    ([xshift=0.6cm, yshift=-0.0cm]vr_head.center) 
    [partial ellipse=170:-170:0.05cm and 0.20cm]
;
\node[black] at ([xshift=0.72cm, yshift=-0.37cm]vr_head.center) {$\beta$};

\draw[black, -{angle 60}] ([yshift=0.38cm]vr_head.center) --++ (90:0.5cm); % z (yaw)
\node[black] at ([xshift=-0.20cm, yshift=0.8cm]vr_head.center) {$z$};
\draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
    ([xshift=0.0cm, yshift=0.5cm]vr_head.center) 
    [partial ellipse=260:-80:0.20cm and 0.05cm]
;
\node[black] at ([xshift=+0.35cm, yshift=0.6cm]vr_head.center) {$\alpha$};

% \node[] (vr_head) at (5.4,3.6)
%     {\includegraphics[width=\imagewidth cm]
%     {figure-journal/mobility-sequence/vr_head.png}
% };

% \draw[black, -{angle 60}] ([xshift=-0.30cm, yshift=-0.30cm]vr_head.center) --++ (-135:0.6cm); % x (roll)
% \node[black] at ([xshift=-0.85cm, yshift=-0.85cm]vr_head.center) {$x$};
% \draw[black, -{stealth[length=1mm,width=1mm]}, rotate=-45] 
%     ([xshift=-0.0cm, yshift=-0.65cm]vr_head.center) 
%     [partial ellipse=440:100:0.25cm and 0.1cm]
% ;
% \node[black] at ([xshift=-0.82cm, yshift=-0.42cm]vr_head.center) {$\gamma$};

% \draw[black, -{angle 60}] ([xshift=0.55cm]vr_head.center) --++ (0:0.6cm); % y (pitch)
% \node[black] at ([xshift=1.3cm, yshift=0.0cm]vr_head.center) {$y$};
% \draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
%     ([xshift=0.8cm, yshift=-0.0cm]vr_head.center) 
%     [partial ellipse=170:-170:0.1cm and 0.25cm]
% ;
% \node[black] at ([xshift=0.85cm, yshift=-0.45cm]vr_head.center) {$\beta$};

% \draw[black, -{angle 60}] ([yshift=0.55cm]vr_head.center) --++ (90:0.6cm); % z (yaw)
% \node[black] at ([xshift=-0cm, yshift=1.3cm]vr_head.center) {$z$};
% \draw[black, -{stealth[length=1mm,width=1mm]}, rotate=0] 
%     ([xshift=0.0cm, yshift=0.8cm]vr_head.center) 
%     [partial ellipse=260:-80:0.25cm and 0.1cm]
% ;
% \node[black] at ([xshift=+0.35cm, yshift=0.6cm]vr_head.center) {$\alpha$};

%%% END: LEGEND %%%


%%% BEGIN: TIME AXIS %%%

%%% Ticks and annotations

\draw[] 
    ([yshift=-(\pitchoffsety+\axisoffsety-0.1)*1cm]ue_upright.center) -- 
    ([yshift=-(\pitchoffsety+\axisoffsety+0.1)*1cm]ue_upright.center);
\node[anchor=north] at 
    ([yshift=-(\pitchoffsety+\axisoffsety+0.1)*1cm]ue_upright.center) {0};

\draw[] 
    ([xshift=-0.5*\imagewidth cm, yshift=-(\pitchoffsety+\axisoffsety-0.1)*1cm]ue_rotated1.center) -- 
    ([xshift=-0.5*\imagewidth cm, yshift=-(\pitchoffsety+\axisoffsety+0.1)*1cm]ue_rotated1.center);
\node[anchor=north] at 
    ([xshift=-0.5*\imagewidth cm, yshift=-(\pitchoffsety+\axisoffsety+0.1)*1cm]ue_rotated1.center) {3};
    
\draw[] 
    ([xshift=0.5*\imagewidth cm, yshift=-(\axisoffsety-0.1)*1cm]ue_pitched.center) -- 
    ([xshift=0.5*\imagewidth cm, yshift=-(\axisoffsety+0.1)*1cm]ue_pitched.center);
\node[anchor=north] at 
    ([xshift=0.5*\imagewidth cm, yshift=-(\axisoffsety+0.1)*1cm]ue_pitched.center) {18};

\draw[] 
    ([yshift=-(\axisoffsety-0.1)*1cm]ue_rotated2.center) -- 
    ([yshift=-(\axisoffsety+0.1)*1cm]ue_rotated2.center);
\node[anchor=north] at 
    ([yshift=-(\axisoffsety+0.1)*1cm]ue_rotated2.center) {33};

\node[anchor=north] at 
    ([xshift=1.3cm, yshift=-(\axisoffsety+0.1)*1cm]ue_rotated2.center) {Time (s)};


%%% Axis itself

\draw[] % Around 0
    ([xshift=-\dotsoffsetx cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_upright.center) --
    ([xshift=\dotsoffsetx cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_upright.center);

\draw[dotted] % 0 to 3
    ([xshift=\dotsoffsetx cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_upright.center) --
    ([xshift=-\dotsoffsetx cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_rotated1.center);

\draw[] % Around 3
    ([xshift=(-0.5*\imagewidth-\dotsoffsetx)*1cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_rotated1.center) --
    ([xshift=(-0.5*\imagewidth+\dotsoffsetx)*1cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_rotated1.center);

\draw[dotted] % 3 to 18
    ([xshift=(-0.5*\imagewidth+\dotsoffsetx)*1cm, yshift=-(\pitchoffsety+\axisoffsety)*1cm]ue_rotated1.center) --
    ([xshift=(0.5*\imagewidth-\dotsoffsetx)*1cm, yshift=-\axisoffsety cm]ue_pitched.center);

\draw[] % Around 18
    ([xshift=(0.5*\imagewidth-\dotsoffsetx)*1cm, yshift=-\axisoffsety cm]ue_pitched.center) --
    ([xshift=(0.5*\imagewidth+\dotsoffsetx)*1cm, yshift=-\axisoffsety cm]ue_pitched.center);

\draw[dotted] % 18 to 33
    ([xshift=(0.5*\imagewidth+\dotsoffsetx)*1cm, yshift=-\axisoffsety cm]ue_pitched.center) --
    ([xshift=-\dotsoffsetx cm, yshift=-\axisoffsety cm]ue_rotated2.center);

\draw[-{angle 60}] % Beyond 33
    ([xshift=-\dotsoffsetx cm, yshift=-\axisoffsety cm]ue_rotated2.center) -- 
    ([xshift=1.5 cm, yshift=-\axisoffsety cm]ue_rotated2.center);

% Movement names
\node[anchor=south] at ([xshift=-1.6 cm, yshift=-\axisoffsety cm]ue_pitched.center) {Yaw};
\node[anchor=south] at ([yshift=-\axisoffsety cm]ue_pitched.center) {Pitch};
\node[anchor=south] at ([xshift=+1.6 cm, yshift=-\axisoffsety cm]ue_pitched.center) {Yaw};

% Snapshot count
\draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex}]
  ([yshift=(-\pitchoffsety-\axisoffsety-\snapshotoffsety)*1cm]ue_upright.center) -- 
  ([yshift=(-\axisoffsety-\snapshotoffsety)*1cm]ue_rotated2.center) 
  node[midway,yshift=-3em] {In total 34 MIMO channel snapshots};
  

%%% END: TIME AXIS %%%

    
\end{tikzpicture}

==> table/panel_tanking.tex <==

\begin{tabular}{>{\rowmac}c||>{\rowmac}c|>{\rowmac}c|>{\rowmac}c|>{\rowmac}c|>{\rowmac}c|>{\rowmac}c|>{\rowmac}c|>{\rowmac}c||>{\rowmac}c>{\rowmac}c|>{\rowmac}c>{\rowmac}c|>{\rowmac}c>{\rowmac}c|>{\rowmac}c>{\clearrow}c}

    \toprule
    
     & \multicolumn{8}{c||}{Employed panels} & \multicolumn{2}{c|}{LoS-HH} & \multicolumn{2}{c|}{LoS-VV} & \multicolumn{2}{c|}{NLoS-HH} & \multicolumn{2}{c}{NLoS-VV} \\
    K & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & P$_{out}$ & q$_{25}$ & P$_{out}$ & q$_{25}$ & P$_{out}$ & q$_{25}$ & P$_{out}$ & q$_{25}$ \\

    \midrule
                        
    \setrow{\bfseries}  1 &   &   & $\times$ &   &   &   &   &   & 18.8 & -47.0 & 23.9 & -48.8 & 32.6 &     / & 74.9 &     / \\
                        1 &   &   &   &   &   &   & $\times$ &   & 23.6 & -48.1 & 44.3 &     / & 33.4 &     / & 65.0 &     / \\ \hline
    
    \setrow{\bfseries}  2 &   &   & $\times$ &   &   &   & $\times$ &   &  2.5 & -38.1 &  9.4 & -42.7 & 13.1 & -46.6 & 47.0 &     / \\
                        2 & $\times$ &   &   &   & $\times$ &   &   &   &  6.0 & -40.8 & 24.3 & -48.9 &  7.6 & -45.6 & 49.6 &     / \\ \hline
                        
    \setrow{\bfseries}  3 &   & $\times$ &   & $\times$ &   &   & $\times$ &   &  0.9 & -35.6 &  5.0 & -40.8 &  4.2 & -43.6 & 33.2 &     / \\
                        3 &   &   & $\times$ &   &   & $\times$ &   & $\times$ &  2.3 & -36.4 &  2.3 & -41.1 &  6.3 & -42.6 & 35.0 &     / \\ \hline
                        
    \setrow{\bfseries}  4 &   & $\times$ &   & $\times$ &   & $\times$ &   & $\times$ &  0.9 & -34.5 &  1.1 & -40.3 &  1.0 & -41.1 & 28.5 &     / \\
                        4 & $\times$ &   & $\times$ &   & $\times$ &   & $\times$ &   &  0.5 & -34.7 &  3.2 & -39.6 &  1.8 & -40.7 & 28.2 &     / \\ \hline
                        
    \setrow{\bfseries}  5 &   & $\times$ & $\times$ & $\times$ &   & $\times$ &   & $\times$ &  0.5 & -33.3 &  0.9 & -39.3 &  0.8 & -40.1 & 26.4 &     / \\
                        5 &   & $\times$ &   & $\times$ &   & $\times$ & $\times$ & $\times$ &  0.9 & -33.8 &  0.9 & -38.8 &  0.8 & -40.6 & 24.5 & -52.2 \\ \hline
                        
    \setrow{\bfseries}  6 &   & $\times$ & $\times$ & $\times$ &   & $\times$ & $\times$ & $\times$ &  0.5 & -32.6 &  0.7 & -37.7 &  0.5 & -39.3 & 23.0 & -49.9 \\
                        6 & $\times$ & $\times$ &   & $\times$ & $\times$ & $\times$ &   & $\times$ &  0.5 & -33.1 &  1.1 & -39.1 &  0.3 & -39.0 & 22.5 & -49.9 \\ \hline
                        
    \setrow{\bfseries}  7 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &   & $\times$ &  0.0 & -31.8 &  0.9 & -38.0 &  0.3 & -38.0 & 20.6 & -49.6 \\
                        7 & $\times$ & $\times$ &   & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &  0.5 & -32.2 &  0.9 & -37.9 &  0.3 & -38.5 & 19.3 & -49.3 \\ \hline
                        
    \setrow{\bfseries}  8 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ &  0.0 & -31.4 &  0.7 & -37.0 &  0.3 & -37.5 & 18.0 & -48.9 \\
     
    \bottomrule
 
\end{tabular}

